Automated Feature Engineering, AutoML, and Decision-Focused Learning for Improved Energy Consumption Forecasting

The rising cost and demand for energy, together with environmental sustainability goals, create major challenges for energy management. Energy Consumption Forecasting (ECF) supports planning by predicting future consumption, but Machine Learning (ML) models for ECF often depend on expert-driven Feature Engineering (FE). This thesis addresses that dependence through three contributions. First, it establishes and evaluates a comprehensive FE pipeline for ECF and investigates domain-specific features. Second, it introduces AutoEnergy, a domain-tailored automated FE algorithm that generates interpretable features from timestamps and lagged consumption and integrates with AutoML for end-to-end ECF modelling. Across eighteen real-world energy datasets spanning residential, commercial, industrial, renewable, and grid domains, AutoEnergy reduces forecasting error by 19.52%-84.72% relative to baseline AutoML and established automated FE methods, while running 1.31-4.41 times faster, with gains varying by dataset. Third, AutoEnergy is integrated with Decision-Focused Learning (DFL) for a Battery Energy Storage System problem, jointly forecasting electricity prices and demand while optimising charging and discharging decisions. On a real-world UK property dataset, this approach reduces operating costs by 22.9%-56.5% compared with the same DFL models without automated FE. Overall, the results show that domain-specific automated FE can reduce reliance on manual feature design, improve forecasting accuracy, and translate predictive gains into measurable operational benefits in energy management.

==> 5-mainChapter/Sections/Pseudocode.tex <==
\label{ch:Pseudocode}


\begin{algorithm}[thpb]
\renewcommand{\thealgorithm}{\(\mathcal{A:}\)}
\captionsetup{font={footnotesize}}
{\caption{Automated Feature Engineering for Energy Consumption Forecasting Problems}
\label{alg:A}
{\footnotesize
\begin{algorithmic}[1] % The [1] option here enables line numbering
\Require DataFrame $D$ with columns $t$ (time stamps) and target variable $y$ (e.g., electricity  consumption)
\Ensure DataFrame $D'$ with new features

\State $D' \gets D$
\State $Features_{time} \gets F_{time}(D, t)$
\State $Features_{cyclical} \gets F_{cyclical}(Features_{time})$
\State $Features_{lags} \gets F_{lags}(D, y)$
\State $Features_{stats} \gets F_{stats}(D, y)$
\State $D' \gets D$ append $Features_{time}$, $Features_{cyclical}$, $Features_{lags}$, $Features_{stats}$

\Function{$F_{time}$}{$D, t$}
    \State $Features_{time} \gets$ Extract time-based features from $t$ {\tiny{\Comment{(e.g., hour of day)}}}
    \State \Return $Features_{time}$
\EndFunction

\Function{$F_{cyclical}$}{$Features_{time}$}
    \State $Features_{cyclical} \gets$ empty list
    \For{feature $f$ in $Features_{time}$}
        \State $f_{sin}, f_{cos} \gets$ Compute $\sin$ and $\cos$ transformations of $f$
        \State Append $f_{sin}, f_{cos}$ to $Features_{cyclical}$
    \EndFor
    \State \Return $Features_{cyclical}$
\EndFunction

\Function{$F_{lags}$}{$D, y$}
    \State $Features_{lags} \gets$ empty list
    \For{$l$ in predefined lags}
        \State $lag\_feature \gets$ shift $y$ by $l$ time units
        \State Compute and append $lag\_feature$ to $Features_{lags}$ if highly correlated with $y${\tiny{\Comment{use Pearson correlation to identify top 10 lags}}}
    \EndFor
    \State \Return $Features_{lags}$
\EndFunction

\Function{$F_{stats}$}{$D, y, Features_{lags}$}
    \State $Features_{stats} \gets$ empty list
    \For{each $lag$ in $Features_{lags}$}
        \State $window \gets lag${\tiny{\Comment{use lag number as a window size}}}
        \State $stat\_features \gets$ Compute rolling window statistics (e.g., mean) of $y$ over $window$
        \State Append $stat\_features$ to $Features_{stats}$
    \EndFor
    \State \Return $Features_{stats}$
\EndFunction
\end{algorithmic}
}}
\end{algorithm}



==> mainchapterorigin/mainchapter.tex <==
\chapter{Main Chapter}
\label{ch:mainchapter}

Main chapter. This can be duplicated several times.

% comment out the following lines if you do not need a table of content for each chapter
% \newpage
% \minitoc % table of content for each chapter
% \newpage

%%%%%%%%%%%
% Figures  
%%%%%%%%%%%
\section{Figures}

Example figure (see Figure~\ref{fig:nottinghamlogo}).

\subsection{Single figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/nottingham-logo.png}
    \caption{Nottingham Logo.}
    \label{fig:nottinghamlogo}
\end{figure}

\subsection{Figures with sub captions}

\begin{figure}[h]
    \centering
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/nottingham-logo.png}
        \caption{Caption A.}
        \label{fig:captiona}
    \end{subfigure}
    \hfill
    \begin{subfigure}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/nottingham-logo.png}
        \caption{Caption B.}
        \label{fig:captionb}
    \end{subfigure}
    \caption{Nottingham Logo.}
\end{figure}

\subsection{Figures side by side}

\begin{figure}[h]
    \centering
    \begin{minipage}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/nottingham-logo.png}
        \caption{Caption C.}
        \label{fig:captionc}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/nottingham-logo.png}
        \caption{Caption D.}
        \label{fig:captiond}
    \end{minipage}
\end{figure}


%%%%%%%%%%%
% Tables  
%%%%%%%%%%%
\section{Tables}

Example table (see Table~\ref{tb:table-example}). 
% Generate LaTeX table quickly with this website: https://www.tablesgenerator.com

\begin{table}[h]
\caption{Table caption.}
\label{tb:table-example}
\begin{tabularx}{\textwidth}{XXX}
\toprule
\textbf{Col 1} & \textbf{Col 2} & \textbf{Col 3} \\ \midrule
\textbf{A}     & 1              & 5              \\
\textbf{B}     & 2              & 6              \\
\textbf{C}     & 3              & 7              \\
\textbf{D}     & 4              & 8              \\ \bottomrule
\end{tabularx}%
\end{table}


%%%%%%%%%%%
% Lists  
%%%%%%%%%%%
\section{Lists}

\subsection{Numbered list}

\subsubsection{Enumeration}

\begin{enumerate}
    \item First item.
    \item Second item.
    \item Third item.
\end{enumerate}

\subsubsection{Research questions}

\begin{enumerate}[font={\bfseries},label={RQ\arabic*}.,align=left]
    \item \rqone
    \item \rqtwo
    \item \rqthree
\end{enumerate}

\subsubsection{Hypothesis}

\begin{enumerate}[font={\bfseries},label={H\arabic*}.,align=left]
    \item First hypothesis.
    \item Second hypothesis.
    \item Third hypothesis.
\end{enumerate}

\subsection{Itemised list}

\begin{itemize}
    \item First item.
    \item Second item.
    \item Third item.
\end{itemize}

\section{Equations}
\begin{equation}
\label{eq:CR}
CR = \frac{(\sum_{i=1}^n \lambda_i)^2}{(\sum_{i=1}^n \lambda_i)^2+(\sum_{i=1}^n \delta_i)} 
\end{equation}
\begin{equation}
\label{eq:AVE}
AVE = \frac{\sum_{i=1}^n \lambda_i^2}{n}
\end{equation}
\begin{equation}
\label{eq:CA}
CA = \frac{n}{n-1}(1-\frac{\sum_{i=1}^n V_i}{V_t}) 
\end{equation}


